Core Challenges of Social Robot Navigation: A Survey

Robot navigation in crowded public spaces is a complex task that requires addressing a variety of engineering and human factors challenges. These challenges have motivated a great amount of research resulting in important developments for the fields of robotics and human-robot interaction over the past three decades. Despite the significant progress and the massive recent interest, we observe a number of significant remaining challenges that prohibit the seamless deployment of autonomous robots in public pedestrian environments. In this survey article, we organize existing challenges into a set of categories related to broader open problems in motion planning, behavior design, and evaluation methodologies. Within these categories, we review past work, and offer directions for future research. Our work builds upon and extends earlier survey efforts by a) taking a critical perspective and diagnosing fundamental limitations of adopted practices in the field and b) offering constructive feedback and ideas that we aspire will drive research in the field over the coming decade.

==> coverletter.tex <==
IJRR

February 27, 2021

Dear Editors,

We wish to submit an original research article entitled “Core Challenges of Social Robot Navigation: A Survey” for consideration by IJRR. We confirm that this manuscript is original and has not been published elsewhere, nor is it currently under consideration for publication elsewhere. 

This article addresses several themes relevant to IJRR through the problem of robot navigation in human environments and the technical challenges associated. The insights presented in this article are key to enabling robots to navigate naturally and safely in human populated environments.  

This article is a survey, reviewing the line of work on this topic over the past three decades. The main narrative of the article is centered around three core technical challenges that we have identified, and the discussions are focused on the papers relevant to those challenges. The social robot navigation problem comprises multiple robotics research areas including robot planning, human-robot interaction, robot learning, and simulation. This article aims to suggest to the interdisciplinary research community possible future research directions to collaboratively address remaining challenges. 

In the submission form, we recommended the following reviewers:
Jonathan How, MIT, USA
Michael Everett, MIT, USA
Kai Arras, Freiburg, Germany
Laurel Riek, UC San Diego, USA
Peter Stone, University of Texas, Austin, USA
Thierry Fraichard, INRIA, France
Takayuki Kanda, Kyoto, Japan
Andrey Rudenko, Orebro, Sweden
Rachid Alami, CNRS, France
Steven Guy, University of Minnesota, USA

To the best of our knowledge, none of these suggested reviewers have any conflict of interest, financial or otherwise.

Thank you for your consideration of this manuscript.

Sincerely,

Jean Oh (Corresponding Author)
The Robotics Institute
Carnegie Mellon University
jeanoh@cmu.edu


==> decoupled-vs-coupled-data-x.tex <==
to make the chart search google scholar in each 1 year period for crowd navigation and social navigation:


1998:
d:
c: 
1999
d:
c: 
2000
d:
c: 
2001
d:
c: 
2002
d:
c: 
2003
d:
c: 
2004
d:
c: 
2005
d:
c: 
2006
d:
c: 
2007
d:
c: 
2008:
d:
c: 
2009:
d:
c: 
2010:
d:
c: 
2011
d:
c: 
2012
d:
c: 
2013
d:
c: 
2014
d:
c: 
2015
d:
c: 
2016
d:
c: 
2017
d:
c: 
2018
d:
c: 
2019


==> input/core-data-challenges-x.tex <==
% !TEX root = ../main.tex
\section{Core Data Challenges of Social Navigation}

In the navigation problem without the social interaction part as defined~\ref{eq:nav}, the primary object of an agent is to reach their destination. Considering this objective only, an agent's navigation performance can be evaluated based on how successful in arriving at a destination, \exempli using the physical distance between an agent's position and a destination. Among the solutions that have reached a destination, it is generally subjective to rank alternatives according to multiple preferences or soft constraints.  Social compliance, for example, is a soft constraint that is comprised of many aspects including safety, comfort, naturalness, and other societal preferences.  
Using a dataset, evaluation is limited to measuring the difference between predictions and the recorded behaviors using a metric such as displacement errors. There are several issues here: 1) recorded behaviors may have been conditioned to a certain context; 2) alternative behaviors that are different from the recording but are equally good can be unfairly penalized; 3) the majority of existing datasets do not have the notion of destinations for the agents in a scene, making it less suitable for a navigation task; 4) recorded behaviors rarely include hard constraint violation such as collision and these rare events need to be engineered/trained based on domain knowledge. 

\subsection{Data Collection}

\textbf{AS}: ``we saw a gap in the existing social navigation datasets. There are datasets that have two, but not all three of the following: natural human motion, robot/human perspective view, and ground truth motion.''

\href{https://docs.google.com/spreadsheets/d/1fS2YJNImJckk6awYaMxi_oUbIBCBm7LThEmTKFDkYU4/edit#gid=0}{\color{blue}\underline{Table of Datasets}}

\subsubsection{Overview of datasets and their characteristics}
\begin{itemize}
    \item A giant table similar to Table 1 in \cite{rudenko2019-predSurvey}.
    
    Characteristics to be included: Indoor/outdoor; Presence of agents other than pedestrians; Presence of robot; Sensors (images, point clouds etc.); top down/perspective view; brief scene description; Labeling (Annotation of groups, annotation of goals; annotation frequency; units (metric/pixel); state representations)
    \item Discussions of usefulness of these characteristics 
\end{itemize}

\subsubsection{How do researchers use these datasets}
\begin{itemize}
    \item Behavior analysis/prediction.
    \item Navigation environments.
\end{itemize}

\subsubsection{Potential metrics for measuring the quality of datasets (or what makes a good dataset)}
\begin{itemize}
    \item time/length
    \item \# of pedestrian tracks
    \item pedestrian density (average / max?)
    \item environment structure/complexity (use entropy to measure?)
    \item interaction diversity (how to measure?)
    \item cultural/geographic diversity
\end{itemize}

\subsection{Problems}


\subsection{Recommendations and Directions for Future Work}

==> input/core-representation-challenges-x.tex <==
\newpage 
\section{Core Representation Challenges of Social Navigation}

\subsection{Representation/Assumption}

Core challenges center around the diversity of ideas/representations/etc for three main tensions. (1) Who is the robot being social with respect to (\exempli how to represent the social agent), (2) whether to handle groups as clusters of individuals or as single group entities, and (3) how to represent and incorporate the influences of the environment

\cmnote{The Social nav section from \citep{thomaz2016computational} has a nice subsection about representations (under a different overall organization) which we could look at to get started.}

\begin{enumerate}[label*=\arabic*.]

	\item{ Entity (Agents/Groups) State
	\begin{enumerate}[label*=\arabic*.]
		\item Raw observation  (e.g. images, point cloud, etc. in end-to-end setting)
		    \begin{itemize}
		        \item DeepMoTIon, end-to-end model, lidar scan to robot action \cite{hamandi19-deepmotion}
		    \end{itemize}
		\item Point (e.g. location, velocity)
		    \begin{itemize}
		        \item NaviGAN and Group-NaviGAN, Location only \cite{tsai20,yao19-group}
		        \item Iterating Gaussian Process (IGP), location only \cite{trautmaniros}
		    \end{itemize}
		\item Pose (e.g. size/shape, orientation, body pose, etc.) 
		    \begin{itemize}
		        \item  Socially Aware - Collision Avoidance Deep Reinforcement Learning (SA-CADRL), state vector has radius and orientation, no longer a dot/point \cite{chen17-sa-cadrl}
		    \end{itemize}
		\item Characteristics and/or Roles (e.g. age, gender, personality, internal state, awareness of other agents, adversary, workflow, etc)
		    \begin{itemize}
		        \item SocioSense, personality model PEN \cite{bera17-sociosense}
		    \end{itemize}
	\end{enumerate}
	}
	
	\item{Group or Individual? 
	\begin{enumerate}[label*=\arabic*.]
		\item Individual
		    \begin{itemize}
		        \item ...
		    \end{itemize}
		\item Group
		    \begin{itemize}
		        \item Group-NaviGAN \cite{yao19-group}
		        \item clustering to make cost maps of groups so system doesn't have to track and plan for every person \cite{Chatterjee1}
		    \end{itemize}
	\end{enumerate}
	}
	
	\item{Modeling Static Environment
	\begin{enumerate}[label*=\arabic*.]
		\item Free space (most of the existing work)
		    \begin{itemize}
		        \item ...
		    \end{itemize}
		\item Traversability/Occupancy (binary map)
		    \begin{itemize}
		        \item ?
		    \end{itemize}
		\item Semantics/Context
		    \begin{itemize}
		        \item ?
		    \end{itemize}
		\item Raw observation (images, point cloud, etc.)
		    \begin{itemize}
		        \item DeepMoTIon, end-to-end model, lidar scan to robot action \cite{hamandi19-deepmotion}
		        \item SoPhie, but it is prediction not navigation \cite{sadeghian19-sophie}; there are a lot of prediction(not navigation) papers use birdview images, PIF, SR-LSTM, etc.
		    \end{itemize}
	\end{enumerate}
	}
\end{enumerate}

\subsection{Recommendations and Directions for Future Work}
\begin{itemize}
    \item Problems
    \item Recommendations
    \item Directions for future work
\end{itemize}


\newpage







% \subsection{How to navigate well}
% \begin{enumerate}[label*=\arabic*.]

% 	\item{ Modeling human environment (?)
% 	\begin{enumerate}[label*=\arabic*.]
% 		\item Obstacle avoidance  (e.g. images, point cloud, etc. in end-to-end setting)
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Uncertainty modeling
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Social rules engineering
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Human processed/inspired (mimicking human behavior)
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Cooperative (topological braid group, etc.)
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
		    
% 	\end{enumerate}
% 	}
	
% 	\item{ How to learn (Source of knowledge on socialness) (?)
% 	\begin{enumerate}[label*=\arabic*.]
% 		\item Reinforcement Learning (exploring by robot itself, e.g. SA-CADRL, SARL)
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Supervised learning / Data driven (from data or demonstration, e.g. NaviGAN, Social Momentum)
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}
% 		\item Non-learning / Rule-based (explicit rules or models asserted by algorithm designers, e.g. IGP, Social Force, etc.) 
% 		    \begin{itemize}
% 		        \item ?
% 		    \end{itemize}

		    
% 	\end{enumerate}
% 	}

% 	\item{ How to assess ``well'' (?)
% 	\begin{enumerate}[label*=\arabic*.]
% 		\item What data to learn from
		 
% 		\item What to evaluate on

% 	\end{enumerate}
% 	}	

% \end{enumerate}


% \subsection{Setting / configuration / Implementation}

% \textcolor{red}{Draft is at \href{https://docs.google.com/document/d/1e53q5wFs2EzXbHeJx7YYMvzPne_gHKuyZmqFUJ08ZU4/edit?usp=sharing}{this google doc}}



==> input/lessons-learned-x.tex <==
% !TEX root = ../main.tex
\section{Lessons Learned and Directions Forward}




\subsection{Evaluation (metrics)} (Eagle, Jean)


\subsection{Interaction modeling} (Chris, ); abstractions of interaction

\subsection{Human expectations and capabilities} (Summary from earlier HRI content, call out key lessons, Allan and Aaron); \exempli appearance-based, tactile sensing, use of language

Cycle time wrt human perception and actuation latencies. Opeions: Incorporate latency into your model, set cycle time low enough to avoid too many operations within human latency, and/or design planner to be robust to latencies in mutual behaviors in other agents.

Humans typically have different fields of view than robots (\exempli wider than Kinect, thinner than 360 lidar). Must account for this when designing for mutual behaviors.

\subsection{Robot Aesthetics}
There is a significant amount of research on the influence of robot appearance on human behavior. For the purposes of this work we want to limit discussion to two aspects that appear to be important for social navigation: robot faces and robot size. 

faces~\cite{kalegina2018-robotface}
%Design, faces or not, design of the Snackbot robot, Multu & Forlizi hospital robot (no face)
%Kanda intercept paper?

size
%Height, ASIMO childlike, Multu paper
%Form Factor (intimidating, childlike, etc), security robots

Because of the wide range of visual design characteristics available to robot developers, we suggest readers explore the rich work in this area for additional insights on the influences of the specific aesthetics present in the robot being used.

\subsection{Environmental context} (Chris)

\subsection{Multiple objectives} multiagents , economy (bounded rationality), game theory

\subsection{Guarantees} formal methods (\exempli Luis Sentis, Peter Stone, U. Texas), safety 

\subsection{Leveraging Attributes of Human Perception}

Take advantage of slower human processing cycle and inaccuracy/noise in human perception. Can be leveraged to use multiple robot processing cycles to improve perception, plans, and predictions. Can also take advantage of more accurate ranging and processing speeds to take action to influence human behavior.

\subsection{Expectations, Skills, Capabilities, and Behaviors of Effective Social Navigation Systems}
\noindent\textbf{Overview} 

What robot behaviors will enable untrained bystanders/pedestrians to navigate effectively around robots? What behavior models and interaction metaphors are most effective for enabling effective robot navigation -- human-like, dog-like, what else?

What social robot navigation performance metrics should we optimize for? How should we measure them? What are appropriate benchmarks? What are some good baselines? How do we ensure that these metrics are accessible to the community?

How do we design social robot navigation studies to address and get beyond novelty effects in our data?

Novelty

\subsection{Abstractions of Social Navigation}
\noindent\textbf{Overview} 

What are the appropriate representations to capture important properties of collective crowd behavior?  

When we abstract away from individual interactions, is fidelity lost?  Does the loss in fidelity justify the (computational?) gains?

What is the right level of detail to include in context models? How does this change depend on the experimental setting?

How do we encode behavior specifications into objective or reward functions?

How do we verify that a robot navigation framework is correct and safe? 

How do we manage a safety critical system without safety guarantees?












==> input/remaining-challenges-x.tex <==
% !TEX root = ../main.tex
\section{Other remaining challenges}\label{sec:other}

\subsection{Robot Design}

While not the direct focus of this work, the robot hardware design is an essential part of accomplishing socially competent robot navigation in human populated environments. Since the early days, roboticists have experimented with a wide variety of robot platforms, featuring a wide range of kinematic models, aesthetics, and anthropomorphic features.

In terms of kinematics, the prevalent paradigm involves wheeled mobile robots with a differential drive. While well-studied and universally available, such robots tend to produce motion that is not humanlike, often confusing humans. Recently, there have been notable alternatives, including the \emph{Ballbot} paradigm \citep{Nagarajan-hri09,Fankhauser_thesis,Lo19}, a robot resembling an inverted pendulum that is dynamically stabilizing on a single point of contact with the floor. Ballbots feature a humanlike form factor and agility that opens up the possibility of smooth merging in densely crowded environments. 

In terms of appearance, many works tend to ignore the aesthetics aspect, focusing on the development of customized functional systems or directly using existing robot platforms. Notably, Rhino \citep{rhino-robot} did not feature any anthropomorphic features but Minerva \citep{minerva-robot}, the second-generation museum guide robot featured a motorized face. Over the following years, many works employed a wide range of platforms with varying levels of humanlikeness, including anthropomorphic features such as a hat \citep{trautman-ijrr-2015} or a virtual face drawn on a screen \citep{Mavrogiannis19}. There is a long and extensive work in HRI literature focusing on the tradeoffs of face design~\citep{DiSalvo02head,kalegina2018-robotface}. Further, it has been shown that the form factor itself is an important aspect of design when it comes to HRI applications~\citep{rae-takayama-mutlu}.

%Broadly, there is a significant amount of research on the influence of robot appearance on human behavior. For the purposes of this work we want to limit discussion to two aspects that appear to be important for social navigation: robot faces~\cite{kalegina2018-robotface} and robot size. 
%Height, ASIMO childlike, Multu paper
%Form Factor (intimidating, childlike, etc), security robots
%Design, faces or not, design of the Snackbot robot, Multu & Forlizi hospital robot (no face)
%Kanda intercept paper?

%Because of the wide range of visual design characteristics available to robot developers, we suggest readers explore the rich work in this area for additional insights on the influences of the specific aesthetics present in the robot being used.

\subsection{Environmental context}
SOPHIE~\cite{sadeghian19-sophie}.

\subsection{Decision making with multiple objectives} multiagents , economy (bounded rationality), game theory

\subsection{Guarantees} 
formal methods (\exempli Luis Sentis, Peter Stone, U. Texas), safety 

\subsection{Leveraging Attributes of Human Perception}

Take advantage of slower human processing cycle and inaccuracy/noise in human perception. Can be leveraged to use multiple robot processing cycles to improve perception, plans, and predictions. Can also take advantage of more accurate ranging and processing speeds to take action to influence human behavior.

\subsection{Expectations, Skills, Capabilities, and Behaviors of Effective Social Navigation Systems}
%\noindent\textbf{Overview} 
Cycle time wrt human perception and actuation latencies. Options: Incorporate latency into your model, set cycle time low enough to avoid too many operations within human latency, and/or design planner to be robust to latencies in mutual behaviors in other agents.

Humans typically have different fields of view than robots (\exempli wider than Kinect, thinner than 360 lidar). Must account for this when designing for mutual behaviors.

What robot behaviors will enable untrained bystanders/pedestrians to navigate effectively around robots? What behavior models and interaction metaphors are most effective for enabling effective robot navigation -- human-like, dog-like, what else?

What social robot navigation performance metrics should we optimize for? How should we measure them? What are appropriate benchmarks? What are some good baselines? How do we ensure that these metrics are accessible to the community?

How do we design social robot navigation studies to address and get beyond novelty effects in our data?

Novelty

% \subsection{Abstractions of Social Navigation}
% %\noindent\textbf{Overview} 

% What are the appropriate representations to capture important properties of collective crowd behavior?  

% When we abstract away from individual interactions, is fidelity lost?  Does the loss in fidelity justify the (computational?) gains?

% What is the right level of detail to include in context models? How does this change depend on the experimental setting?

% How do we encode behavior specifications into objective or reward functions?

% How do we verify that a robot navigation framework is correct and safe? 

% How do we manage a safety critical system without safety guarantees?












==> keywords.tex <==
Keyword list:

Social Human-Robot Interaction < Human-centered and Life-like Robotics	 

Cognitive Human-Robot Interaction < Cognitive Robotics	 

Learning and Adaptive Systems < Cognitive Robotics	 

Path Planning for Multiple Mobile Robot Systems < Mobile and Distributed Robotics SLAM	 

Autonomous Agents < Cognitive Robotics	
 


==> notes.tex <==
Bibliography (Eagle, Allan)
- Pete's (included here) -- upto 2015 (sparse after 2012); no interaction
- Chris's .bib (thesis done in 2019); representation, context
- Marynel's (); interaction, environmental context (modeling human body orientation, POMDPs)
https://www.ri.cmu.edu/publications/reasoning-about-spatial-patterns-of-human-behavior-during-group-conversations-with-robots-2/ 
- Andy's MS thesis 2019, RL/IRL 
- Chatterjee's MS thesis (group perception, Gestalt) 
- Allan's paper
6/18 -- a full list compiled.

Labels for tagging papers:
- irrelevant
- general, e.g., 


Avoid overlap
- Prediction survey 2019
- Simulation survey

Problem formulation
- Everyone will take a look and add/edit/drop 

Lessons learned + future directions
- Keep updating the list

ORCID
Chris: https://orcid.org/0000-0003-4476-1920
Francesca: https://orcid.org/0000-0003-2296-5762
Allan: https://orcid.org/0000-0002-8253-2742
Eagle: https://orcid.org/0000-0003-2136-0198
Pete: https://orcid.org/0000-0002-9793-7697
Aaron: https://orcid.org/0000-0003-2274-0053
Jean: https://orcid.org/0000-0001-9709-2658



